An Efficient Cyclic Entailment Procedure in a Fragment of Separation Logic

An efficient entailment proof system is essential to compositional verification using separation logic. Unfortunately, existing decision procedures are either inexpressive or inefficient. For example, Smallfoot is an efficient procedure but only works with hardwired lists and trees. Other procedures that can support general inductive predicates run exponentially in time as their proof search requires back-tracking to deal with a disjunction in the consequent. This paper presents a decision procedure to derive cyclic entailment proofs for general inductive predicates in polynomial time. Our procedure is efficient and does not require back-tracking; it uses normalisation rules that help avoid the introduction of disjunction in the consequent. Moreover, our decidable fragment is sufficiently expressive: It is based on compositional predicates and can capture a wide range of data structures, including sorted and nested list segments, skip lists with fast forward pointers, and binary search trees. We have implemented the proposal in a prototype tool and evaluated it over challenging problems taken from a recent separation logic competition. The experimental results confirm the efficiency of the proposed system.

==> algo-pred2base.tex <==
\begin{algorithm2e}[t]
  \SetKwInOut{Input}{input}\SetKwInOut{Output}{output}
  \SetAlgoLined

 \Input{$\PName$} \Output{$\code{base}^{\PName}$}
   \ForEach{$\seppred{\code{P_i}}{\setvars{t}_i} \in \PName$}{%
      $\form{(V, E, \backfun)} {\leftarrow}$ {\allSat}$(\seppred{\code{P_i}}{\setvars{t}_i})$ \tcc*{reduction tree}
     $\Psi \leftarrow \{ \textcolor{blue}{\D^{noncyc}_{{\sat}}} \mid 
 \textcolor{blue}{(\D^{noncyc}_{{\sat}})^N} \text{ is {\sat}} \}$ \tcc*{{\sat} leaf nodes $\notin$ cycles}
     \ForEach{$\text{outer } \form{\ctree{N_c}{N_b}{\sub}} $}{
       $\Psi^S \leftarrow \emptyset$ \;
       $\atom \leftarrow  \bigvee \{Pres(N_{b_i}^N)\}$ \tcc*{arithmetic of buds}
       \ForEach{ $ \textcolor{blue}{\D_{\sat}} \in \form{\ctree{N_c}{N_b}{\sub}} $}{
         $\Psi^S \leftarrow \Psi \cup \{ \D_{\sat}^S\} $ \tcc*{spatial projection of {\sat} leaf nodes}
         $\atom \leftarrow \atom {\vee} Pres(\D_{\sat}^N)$ \tcc*{arithmetic of {\sat} leaf nodes}
       }
       $\Psi \leftarrow \Psi \cup \{\base \wedge \atom \mid \base \in \Psi^S  \}$ \;
     }

     $\basep{(\seppred{\code{P_i}}{\setvars{t}_i})}  {\leftarrow} \Psi $\;
    }
  \Return{$\code{base}^{\PName}$};
 \caption{Deriving Bases.}\label{algo.singleton.base}
\end{algorithm2e}


==> fig-shlid.tex <==
\begin{figure}[tb]
\begin{center}
\[
\begin{array}{l}
 \seppred{\code{pred~sll}}{r{,}F} ~{\equiv}~ \emp {\wedge} r{=}F ~ \vee ~ \exists {X_{tl}}.
 \sepnode{r}{c_1}{X_{tl}} {\sep} \seppred{\code{sll}}{X_{tl},F} {\wedge} r{\neq}F\\
 \seppred{\code{pred~nll}}{r{,}F{,}B} ~{\equiv}~ \emp {\wedge} r{=}F \\
 ~\quad \vee ~ \exists {X_{tl}}{,}Z.
 \sepnode{r}{c_2}{Z,X_{tl}} {\sep}  \seppred{\code{sll}}{Z,B}{\sep} \seppred{\code{nll}}{X_{tl},F,B} {\wedge} r{\neq}F {\wedge} r{\neq}B \\
 \seppred{\code{pred~skl1}}{r{,}F} ~{\equiv}~ \emp {\wedge} r{=}F
 ~ \vee ~ \exists {X_{tl}}.
 \sepnode{r}{c_3}{X_{tl}{,}\nil{,}\nil} {\sep}  \seppred{\code{skl1}}{X_{tl},F} {\wedge} r{\neq}F  \\
\seppred{\code{pred~skl2}}{r{,}F} ~{\equiv}~ \emp {\wedge} r{=}F \\
 \quad~ \vee ~ \exists {X_{tl},Z_1}.
 \sepnode{r}{c_3}{Z_1{,}X_{tl}{,}\nil} {\sep} \seppred{\code{skl1}}{Z_1{,}X_{tl}} {\sep}  \seppred{\code{skl3}}{X_{tl},F} {\wedge} r{\neq}F  \\
 \seppred{\code{pred~skl3}}{r{,}F} ~{\equiv}~ \emp {\wedge} r{=}F \\
 \quad~ \vee ~ \exists {X_{tl},Z_1,Z_2}.
 \sepnode{r}{c_3}{Z_1{,}Z_2{,}X_{tl}} {\sep} \seppred{\code{skl1}}{Z_1{,}Z_2} {\sep}  \seppred{\code{skl2}}{Z_2{,}X_{tl}} {\sep}  \seppred{\code{skl3}}{X_{tl},F} {\wedge} r{\neq}F  \\
\end{array}
\]
\caption{{\csl} Predicate Definitions.}
\label{fig.shlid}
\end{center}
\end{figure}


==> fig-sl-sem.tex <==
\begin{figure}[tb]
\begin{center} %%\savespace %% \savespace
%\begin{minipage}{0.98\textwidth}
%\begin{frameit} \savespace  %\savespace
\hide{\[
\begin{array}{lcl}
 \form{\sstack} \force \pure_1 {\wedge} \pure_2 & \iffs &
 \form{\sstack} \force \pure_1 \text{ and }
 \form{\sstack}\force \pure_2 \\
\form{\sstack} \force \pure_1 {\vee} \pure_2 & \iffs &
 \form{\sstack} \force \pure_1 \text{ or }
 \form{\sstack}\force \pure_2 \\
 \form{\sstack} \force v_1{\oslash}v_2 & \iffs & \force {\sstack}(v_1)~{\oslash}~ {\sstack}(v_2) \text{, where }
 \oslash \in \{=,\neq\}
  \\
 \form{\sstack} \force {\a_1}{\oslash}{\a_2} & \iffs & \force {\sstack}(\a_1)~{\oslash}~ {\sstack}(\a_2) \text{, where }
 \oslash \in \{=,\leq\}
  \\
 %% \form{\sstack} \force {\bag_1}{\oslash}{\bag_2} & \iffs & \force {\sstack}(\bag_1)~{\oslash}~ {\sstack}(\bag_2) \text{, where }
 %% \oslash \in \{\in,=,{\bagsubsume},  {\bagunion},{\bagintersect},{\bagsubtract} \}
 %%  \\
 \end{array}
 \]}
 \[
 \begin{array}{lcl}
\form{\sstack},\form{\sheaps} \force \emp &
\iffs & \sheaps {=} \emptyset\\
\form{\sstack},\form{\sheaps} \force \sepnodeF{v}{c}{f_i:v_i} &
%% iffs &  l {=}\sstack(v), \text{dom}(\sheaps) {=}\{l \rightarrow r \}
%% \mbox{ and } r(c,f_i){=} \sstack({v_i})\\
\iffs &  \text{dom}(\sheaps) {=}\{\sstack(v)\}
\mbox{ and } \sheaps(\sstack(v), c,f_i){=} \sstack({v_i})\\
%% \form{\sstack},\form{\sheaps} \force \seppredF{\code{p}}{\setvars{v}} &
%% \iffs & (\form{\sstack(\setvars{v}),}\form{\sheaps}) \in \text{\textlbrackdbl} \seppredF{\code{p}}{\setvars{v}} \text{\textrbrackdbl} \\
%%
\form{\sstack},\form{\sheaps}  \force \seppredF{\code{P}}{\setvars{t}} & \iffs &
\form{\sstack},\form{\sheaps} \force \form{\seppredF{\code{P}}{\setvars{t}}^m} \text{ for some } \form{m{\geq}0}\\
\form{\sstack},\form{\sheaps}  \force \seppredF{\code{P}}{\setvars{t}}^{k{+}1} & \iffs &
\form{\sstack},\form{\sheaps}  \force \form{\D[\seppredF{\code{P}}{\setvars{t}}^{k}/P(\setvars{t})]} \text{ for some definition branch } \D \text{ of \code{P}} \\
\form{\sstack},\form{\sheaps} \force \seppredF{\code{P}}{\setvars{t}}^0  & \iffs & \mbox{never}\\
%
%\end{array}
%&
%\begin{array}{lcl}
\form{\sstack},\form{\sheaps} \force  \heap_1 \sep \heap_2 &
\iffs & \exists \sheaps_1,\sheaps_2 {\cdot}~ \sheaps_1 {\#} \sheaps_2 \mbox{ and }
 \sheaps{=}\sheaps_1 {\cdot} \sheaps_2 \mbox{ and }
 \sstack,\sheaps_1 \force \heap_1 \mbox{ and } \sstack,\sheaps_2 \force \heap_2\\
%%%%%%%%%%%
%% \form{\sstack},\form{\sheaps} \force  \heap_1 \wedge \heap_2 &
%% \iffs & \sstack,\sheaps \force \heap_1 \mbox{ and } \sstack,\sheaps \force \heap_2\\
%%%%%%%%%%%%%%%%
%\end{array}
%% \end{array}
%% \]
%% \[
%% %% \begin{array}{ll};
%% \begin{array}{lcl}
\form{\sstack},\form{\sheaps} \force \true &
\iffs & \mbox{always} \qquad \qquad \qquad \form{\sstack},\form{\sheaps} \force \false \quad  \iffs \quad  \mbox{never}\\
%% \form{\sstack},\form{\sheaps} \force \false &
%%  \iffs & \mbox{never}\\
\form{\sstack},\form{\sheaps} \force \exists {v} {.}(\heap{\wedge}\pure) &
\iffs & \exists {\alpha} \cdot {\sstack}[v \pto {\alpha}],\form{\sheaps} \force {\heap}  \text{ and } {\sstack}[v \pto {\alpha}] \force {\pure} \\
%% \form{\sstack},\form{\sheaps} \force \neg \constr &
%% \iffs & \form{\sstack},\form{\sheaps} \nforce \constr \\
\form{\sstack},\form{\sheaps} \force  \constr_1 \vee \constr_2 &
\iffs & \sstack,\sheaps \force \constr_1 \mbox{ or } \sstack,\sheaps \force \constr_2\\
\end{array}
\]
%\end{frameit}
%\vspace{-5pt} \savespace
%\end{minipage} \saveone
\caption{Semantics.} %% with Precise Assertions \cite{Reynolds:08}.}
\label{fig.sl.sem}
\end{center}
\savespace
 \savespace
\end{figure}


==> fig-sl-syn.tex <==
 \begin{figure}[tb]
 \begin{center}
 \[
\begin{array}{ll}
\begin{array}{l}
\textit{Pred} ::= \seppred{\code{pred~P_i}}{\setvars{v}_i}  {\equiv} \constr_i;
\\
\constr ::= \D ~|~ \constr_1 ~{\vee}~ \constr_2
\qquad  ~ \D ::= \exists \bar{v}{.}~(\heap{\wedge}\pure)
 \\
 \heap ::= \emp ~|~ % \topF ~|~
\sepnodeF{x}{c}{f_i{:}v_i} ~|~
\seppredF{\code{P}}{\setvars{v}}
~|~\heap_1 {\sep}\heap_2 \\
% \text{Pure formula} &
 \pure ::=  \true |
   \atom | \phi | {\neg} \pure_1 |
\exists v{.}~\pure \mid
\pure_1 {\wedge} \pure_2 \\
\end{array}
&\quad
\begin{array}{l}
\textit{Node} ::= \code{data}~ c_i \{\tau_1 ~ f_{i_1};..;\tau_j~f_{i_j} \} \\
\phi ::=  v_1 {=}v_2 | v{=}\nil  \quad \tau ::= \code{Int} \mid c \\
\atom ::=   \a_1 {=} \a_2 \mid \a_1 {\leq} \a_2 \\
 a ::= \!k \mid v \mid k {\times}\a \mid \a_1 \!+\! \a_2 \mid - \a
\end{array}
\end{array}
\]
\caption{Syntax}\label{prm.spec.fig}
\end{center}
\end{figure}


==> pred-dpi.tex <==
%%\paragraph{DPI periodic predicates \cite{Makoto:APLAS:2016}}
In consequence, we define %% a class of flattable formulas,
%% called flat
DPI formula, based on
%% bounded
DPI predicates where each predicate
is equivalent to a Presburger formula \cite{Makoto:APLAS:2016}.

An arithmetic inductive predicate is DPI if it is not inductive or is defined as follows.
\[
\begin{array}{l}
\code{pred}~ P^N(\setvars{x}) \equiv \bigwedge_{1 \le i \le m} \phi_{0,i}
\vee
\exists \setvars{z}\cdot \bigwedge_{1 \le i \le m} \phi_i \land \bigwedge_{1 \le l \le L}
 P^N(\setvars{z}^l)
\end{array}
\]
where
$m$ is the arity of $P^N$,
$\FV(\phi_{0,i}) {\subseteq} \{ x_i \}$,
$\setvars{z} {\supseteq} \setvars{z}^l$, and
there exists $j$ such that
$\phi_i$ is either of
$x_i {=} f(\setvars{z}_i)$,
$x_i {\ge} f(\setvars{z}_i)$,
or 
$x_i {\le} f(\setvars{z}_i)$
for all $i {\ne} j$,
and
$\phi_j$ is either of the following:
\[
\begin{array}{l}
\begin{array}{lll}
(1)~ \form{x_j = f(\setvars{z}_j) + c \land \phi'} &\qquad
(2)~ \form{x_j \ge f(\setvars{z}_j) + c \land \phi'}&\qquad
(3)~ \form{x_j \le f(\setvars{z}_j) + c \land \phi'} \\
\end{array} \\
{}\\
(4) \text{ a conjunction of the following forms with some integer constant }
 \form{n>0}:\\
\qquad \form{\phi'}, \form{n x_j = f(\setvars{z}_j)},
 \form{n x_j \ge f(\setvars{z}_j)},or ~\form{n x_j \le f(\setvars{z}_j)}
\end{array}
\]
where
$c$ is some integer constant,
$\setvars{z}_j$ is $z_j^1,\ldots,z_j^L$,
$\phi'$ is an arithmetical formula such that $\FV(\phi') \subseteq \setvars{z}_j$
and $\phi'[z/\setvars{z}_j]$ is true for any $z$,
$f(\setvars{z}_j)$ is
a combination of $z_j^1,\ldots,z_j^L$ with $\max,\min$,
defined by
\form{
f(\setvars{z}_j) ::= z_j^l \ |\  \max(f(\setvars{z}_j), f(\setvars{z}_j)) \ |\  \min(f(\setvars{z}_j), f(\setvars{z}_j))},
and $f$'s may be different from each other in the conjunction of (4).

%% Note that each inductive definition in DPI has at most one induction case and mutual inductive definitions are not allowed.
The authors in \cite{Makoto:APLAS:2016} showed that each inductive predicate DPI exactly represents some eventually periodic sets
which are equivalent to some sets characterized by some Presburger arithmetical formulas.
\begin{lemma}[\cite{Makoto:APLAS:2016}]\label{lem.dpi}
For every DPI inductive predicate $P(\setvars{x})$, there is
a formula $\phi$ equivalent to $P(\setvars{x})$ such that
$\phi$ does not contain any inductive predicates.
\end{lemma}


==> proj.tex <==
 The following definition is critical for the computation of base formulas.

%% In this subsection,
%% We define numeric  and
%%  spatial
%%  projection functions.
%% The numeric projection is critical for computing
%% the base.
%% of a predicate.
%% For each predicate \form{\code{P} \in \PName}
%% we assume there exist predicate
%% \code{P^N} (resp. \code{P^S}) for its numeric (resp. spatial) projection.
%% Similarly,
%% For each \form{c \in {\Dns}}, we assume
%% node symbol \code{c^N} %% (resp. \code{c^S})
%% for its numeric %% (resp. spatial)
%% projection.
%% \code{c^S} is a sequence of fields similarly to \form{c}
%% except that non-pointer fields are replaced by the \form{\_} fields.
For each \form{c \in {\Dns}}, 
we assume \code{c^N} is a sequence of fields similarly to \form{c}
except that pointer-typed fields are replaced by the \form{\_} fields.
%
Similarly, we assume
node symbol \code{c^S}
for its  spatial
projection.
\code{c^S} is a sequence of fields similarly to \form{c}
except that non-pointer fields are replaced by the \form{\nil} fields.

The spatial projection
$(\constr)^S$ is defined inductively:
\[
\begin{array}{ll}
\begin{array}{lcl}
\form{(\D_1 \vee \D_2)^S} & \equiv &
 \form{(\D_1)^S} \vee \form{(\D_2)^S} \\
\form{(\exists \setvars{x}. \D)^S} & \equiv &
 \form{\exists \setvars{x}^S . (\D)^S} \\
\form{(\heap{\wedge}\atom{\wedge}\phi)^S} & \equiv &
\form{(\heap)^S{\wedge}\atom} \\
\end{array} & \qquad
\begin{array}{lcl}
\form{(\heap_1 {\sep} \heap_2)^S} & \equiv &
\form{(\heap_1)^S} {\sep} \form{(\heap_2)^S} \\
\form{(\seppredF{\code{P}}{\setvars{v}})^S} & \equiv &
\seppredF{\code{P^S}}{\setvars{v}^S} \\
\form{(\sepnodeF{x}{c}{\setvars{v}})^S}  & \equiv & \form{\sepnodeF{x}{c^S}{\setvars{v}^S}} \quad
\form{(\emp)^S}  \equiv  \emp \\
\end{array}
\end{array}
\]
%\end{defn}
%
For each inductive predicate \form{\seppred{\code{P}}{\setvars{t}}{\equiv}\constr},
 we assume the inductive predicate symbols
\code{P^S} and predicate \seppred{\code{P^S}}{\setvars{t}^S}
for its spatial projection satisfy \form{\seppred{\code{P^S}}{\setvars{t}^S} {\equiv} \constr^S}.



%% The semantics of the  projection \seppred{\code{P^S}}{\setvars{t}^S} is
%% as follows. Let \form{\sbase_P} be a (infinite)
%%  set base formulas derived from
%%  \form{\seppred{\code{P}}{\setvars{t}}}.
%% If all variables in \form{\setvars{t}} are numeric-typed, then
%% \form{\seppred{\code{P^S}}{\setvars{t}^s}{\equiv} \true}.
%% Otherwise,
%% \form{\seppred{\code{P^S}}{\setvars{t}^S} {\equiv} \bigvee \{(\base)^S \mid \base \in \form{\sbase}_P \} }.

%% The spatial projection of predicate
%% \form{
%% \defpred~ \seppred{\code{P}}{\setvars{t}}  ~{\equiv}~
%%    \bigvee^n_{i=1} ({\exists} \setvars{w_i}{\cdot}~ \D_i:l_i);
%% } is defined as
%%  \form{
%% \defpred~ \seppred{\code{P}^S}{\setvars{t}^S}  ~{\equiv}~
%%    \bigvee^n_{i=1} ({\exists} \setvars{w_i}{\cdot}~ \D_i)^S:l_i;
%% }.

%% For examples, the spatial projections of predicates \code{P}, \code{Q}
%% are as follows.
%% \[%%\savespace
%% \begin{array}{l}
%% \code{pred}~\form{\seppred{\code{P}^S}{x} \equiv
%%   x{=}\nil: 0}
%% ~~{\vee}~ \form{~ \seppred{\code{Q}^S}{x{,}x}{\wedge}x{\neq}\nil:1}; \\
%% \code{pred}~\form{\seppred{\code{Q}^S}{x{,}y} \equiv
%% {\exists} ~x_1{,}y_1 {\cdot}\sepnode{x}{node}{x_1,y_1}{\sep} \seppred{\code{P}^S}{x_1}\wedge y{=}\nil{\wedge}x{\neq}\nil:0}
%%  \\
%% ~~~ {\vee}~ \form{~{\exists} ~x_1{,}y_1 {\cdot} \sepnode{y}{node}{x_1{,}y_1} \sep
%% \seppred{\code{Q}^S}{x,y_1}{\wedge}y{\neq}\nil:1} ;\\
%% \end{array}
%% \]

%
%\begin{defn}%%[Numeric Projection]
\label{defn.numeric.proj}
The numeric projection
$(\constr)^N$ is defined inductively as follows.
\[
\begin{array}{ll}
\begin{array}{lcl}
\form{(\D_1 \vee \D_2)^N} & \equiv & \form{(\D_1)^N} \vee \form{(\D_2)^N} \\
\form{(\exists \setvars{x} \cdot \D)^N} & \equiv &
 \form{\exists \setvars{x}^N \cdot (\D)^N} \\
\form{(\heap{\wedge}\atom{\wedge}\phi)^N} & \equiv &
\form{(\heap)^N{\wedge}\phi} \\
\end{array} & \qquad
\begin{array}{lcl}
\form{(\heap_1 {\sep} \heap_2)^N} & \equiv &
\form{(\heap_1)^N} {\wedge} \form{(\heap_2)^N} \\
 \form{(\seppredF{\code{P}}{\setvars{v}})^N} & \equiv &
 \seppredF{\code{P^N}}{\setvars{v}^N} \\
\form{(\sepnodeF{x}{c}{\setvars{v}})^N}  {\equiv}
\form{(\emp)^N} & \equiv & \true \\
\end{array}
\end{array}
\]
%\end{defn}
For each inductive predicate \form{\seppred{\code{P}}{\setvars{t}}{\equiv}\constr},
 we assume the inductive predicate symbols
\code{P^N} and predicate \seppred{\code{P^N}}{\setvars{t}^N}
for its numeric projection satisfy \form{\seppred{\code{P^N}}{\setvars{t}^N} {\equiv} \constr^N} if \form{\constr} does not contain
any occurrence of other inductive predicates.
If it contains an occurrence of predicate \form{\seppredF{\code{Q}}{\setvars{v}}} then the numeric project of \code{Q} is computed by:
 \form{\seppredF{\code{Q}^N}{\setvars{v}}^N \equiv \bigvee\{(\base)^N \mid \base \in \basep{\seppredF{\code{Q}}{\setvars{v}}} \}}.
%% The semantics of the numeric projection \seppred{\code{P^N}}{\setvars{t}^N} is
%% as follows. Let \form{\sbase_P} be a (infinite)
%%  set base formulas derived from
%%  \form{\seppred{\code{P}}{\setvars{t}}}.
%% If all variables in \form{\setvars{t}} are pointer-typed, then
%% \form{\seppred{\code{P^N}}{\setvars{t}^N}{\equiv} \true}.
%% Otherwise,
%% \form{\seppred{\code{P^N}}{\setvars{t}^N} {\equiv} \bigvee \{(\base)^N \mid \base \in \form{\sbase}_P \} }.
%% For a syntactic projection, we add the following rule
%% for predicate instance:
%%  \form{(\seppredF{\code{P}}{\setvars{v}})^N  \equiv
%%  \seppredF{\code{P^N}}{\setvars{v}^N}}. Then,
%% the definition of the arithmetic is defined as:
%% \form{\seppred{\code{P^N}}{\setvars{t}^N} {\equiv} \constr^N}.
%%  of  of predicate
%% \form{
%% \defpred~ \seppred{\code{P}}{\setvars{t}}  ~{\equiv}~
%%    \bigvee^n_{i=1} ({\exists} \setvars{w_i}{\cdot}~ \D_i:l_i);
%% } is defined as
%%  \form{
%% \defpred~ \seppred{\code{P}^N}{\setvars{t}^N}  ~{\equiv}~
%%    \bigvee^n_{i=1} ({\exists} \setvars{w_i}{\cdot}~ \D_i)^N:l_i;
%% }.
\hide{For examples, the numeric projections of predicates \code{P}, \code{Q}
are as follows.

\[%%\savespace
\begin{array}{l}
\code{pred}~\form{\seppred{\code{P}^N}{n} \equiv
  {n{=}0: 0}}
~~{\vee}~ \form{~{\exists}n_1 {\cdot} \seppred{\code{Q}^N}{n_1}{\wedge} n{=}n_1:1}; \\
\code{pred}~\form{\seppred{\code{Q}^N}{n} \equiv
{\exists} ~n_1 {\cdot \seppred{\code{P}^N}{n_1}{\wedge}{n{=}n_1{+}1:0}}}
 \\
~~~ {\vee}~ \form{~{\exists} ~n_1 {\cdot}
\seppred{\code{Q}^N}{n_1}{\wedge}n{=}n_1{+}1:1} ;\\
\end{array}
\]}

%% \begin{theorem}
%% For all \form{\sstack}, \form{\sheaps} s.t.
%% \form{\sstack{,}\sheaps \force \constr} iff
%%  \form{\sstack{,}\sheaps \force (\constr)^S}
%% and \form{\sstack \force (\constr)^N}
%% \end{theorem}
%% While the proof of the ``if" direction is straightforward,
%% the proof of the ``only if" can be done by structural induction.


==> syntax-local.tex <==
%\paragraph{Semantic Local Properties}
%\input{fig-sat-small}
%% Next, we define {\shide} by augmenting additional parameters into  {\csl} predicates to capture elastic properties.
We discuss semantics of
the local properties where our decidable fragment is based on.
Intuitively,
a local property specified over a (infinite) set of objects
is an universally quantified invariant over the set.
Especially, the validity of such invariant
could be checked locally
through a group of a  small number of objects.
In this work, we consider three local properties: injectivity, transitivity
and order.

\noindent{\bf Injectivity}
The  injectivity property is used to specify additional links of
a data structure
e.g., singly-linked lists with an
 additional link to capture {\em previous} pointer
 of each node (e.g., doubly-linked lists
or trees with parents-pointers). %%  For instance, we extend predicate \form{sll}
%% to obtain doubly-linked lists as follows.
%% \[
%% \begin{array}{l}
%% \seppred{\code{pred~dll}}{r{,}F{,}pr{,}lst} ~{\equiv}~ \emp {\wedge} r{=}F {\wedge}lst{=}pr\\
%% \qquad \exists X_{tl}. \sepnode{r}{c_2}{pr{,}X_{tl}} \sep \seppred{\code{dll}}{X_{tl}{,}F{,}r{,}lst} {\wedge} r{\neq}F
%% \end{array}
%% \]
Supposed predicate \form{\seppred{\code{P_i}}{\setvars{v}_i}} be universally
quantified by an injectivity property through two fields \form{f_i} and \form{f_j}
of a heap structure \form{c}, then
 for any \form{\sstack, \sheaps},
 we have:
  \[
\text{ if } \form{\sstack, \sheaps \force \seppred{\code{P_i}}{\setvars{v}_i}},
 \forall l_1 \in \dom(h). \exists ~ l_2 \in  \dom(h). h(l_1, c, f_i) = l_2 \text{ then }
h(l_2, c, f_j) {=}l_1.
\]

\noindent{\bf Transitivity}
The transitivity property
is used to specify a constant data content at field \form{f_j} of every heap cells in a predicate.
For an instance, it is used to specify
 singly-linked lists
where  every singleton heaps contains the same value \form{a}, %% (e.g., the predicate \code{slla} defined below),
or singly-linked lists whose every node points-to the last node.
%% \[
%% \begin{array}{l}
%% \seppred{\code{pred~slla}}{r{,}F{,}s{,}t} ~{\equiv}~ \emp {\wedge} r{=}F  {\wedge}s{=}t \\
%% \qquad \exists X_{tl}. \sepnode{r}{c_2}{X_{tl}{,}s} \sep \seppred{\code{slla}}{X_{tl}{,}F{,}s{,}t}  {\wedge} r{\neq}F \\
%% \end{array}
%% \]
Supposed predicate \form{\seppred{\code{P_i}}{\setvars{v}_i,x,t}} be universally
quantified by a transitivity property through a field \form{f_j}
of a heap structure \form{c}, then
 for any \form{\sstack, \sheaps},
 we have:
  \form{
\text{ if } \form{\sstack, \sheaps \force \seppred{\code{P_i}}{\setvars{v}_i,x,t}},
\text{ then } \forall l_1 \in \dom(h). h(l_1, c, f_j) =  \sstack(x)
}.

\noindent{\bf Order}
The order property is used to specify sortedness of a predicate e.g., singly-linked lists
being sorted %% (e.g., predicate \code{sllso} defined below)
or trees being binary search trees.
%% \[
%% \begin{array}{l}
%% \seppred{\code{pred~sllso}}{r{,}F{,}mi{,}ma} ~{\equiv}~ \emp {\wedge} r{=}F {\wedge}ma{=}mi \\
%% \qquad \exists X_{tl}{,}mi_1. \sepnode{r}{c_4}{mi{,}X_{tl}} \sep \seppred{\code{sllso}}{X_{tl}{,}F{,}mi_1{,}ma} {\wedge} r{\neq}F \wedge mi {<} mi_1
%% \end{array}
%% \]
Supposed predicate \form{\seppred{\code{P_i}}{\setvars{v}_i}} be universally
quantified by an order property such that heap cells of the predicate is linked
by a field \form{f_j} (of a heap structure \form{c}) and their
data content at a field \form{f_j} are sorted, then
 for any \form{\sstack, \sheaps}, %% \form{p} is an instance of \form{P_i},
 we have (where
  \form{\diamond \in \{=,\geq, \leq\}}):
  \[
  % \form{p\neq \nil \wedge p.{f_i}\neq \nil, \text{ then }  p.f_i.f_j < p.f_j }
\text{ if } \form{\sstack, \sheaps \force \seppred{\code{P_i}}{\setvars{v}_i}},
 \forall l_1 {\in} \dom(h). \exists l_2 {\in}  \dom(h). h(l_1{,} c{,} f_i) {=} l_2 \text{ then }
h(l_1{,} c{,} f_j) \diamond h(l_2{,} c{,}f_j).
\]

\begin{remark}[Cyclic proofs with local properties]
We restrict the pure formula over these local properties as
these properties help ensure the termination of our entailment procedure.
That is,
given an entailment,
the proposed procedure terminates
iff it terminates
over the projection without these local properties.
\end{remark}






==> tbl-entl.tex <==
%% \begin{table}[tb]
%% %\small
%% \begin{center}
%% \caption{Experimental Results on Entailment} \label{tbl:expr.entl}
%% \begin{tabular}[t]{|c|c  | c | c |c | c| c| c |c | c | c|c|c|c|c|}
%% \hline
%%              &   \multicolumn{2}{c|}{\#problem} & \multicolumn{2}{c|}{({\invalid})\#$\surd$} & \multicolumn{2}{c|}{({\valid})\#$\surd$}& \multicolumn{2}{c|}{Time} \\
%% \hline
%%    Div. & \#{\small \invalid} &  \#{\small \valid} &  {\songbird}& \toolname   & {\songbird} & \toolname   & {\songbird} & \toolname \\
%% \hline
%% shls & 122 & 174 & 12 & 122 & 174 &  174 & 237m25s & 17.01s \\
%% \rowcolor{Gray}shlid & 24 & 36 & 2 & 24 & 36 & 36  & 40m38s & 3.94s \\
%% shidlia & 8 & 67 & 0 & 0 & 24 & 12  & 183m41s & 220m9s \\
%% \hline
%%  \end{tabular}
%% \end{center}
%% \end{table}
\begin{table}[tb]
%\small
\begin{center}
\caption{Experimental Results on Entailments} \label{tbl:expr.entl}
\begin{tabular}[t]{|c|c  | c | c |c  | c | c |c  | c | c |}
\hline
 Tool            &   \multicolumn{3}{c|}{{\em qf\_shls\_entl}} &   \multicolumn{3}{c|}{{\em qf\_shlid\_entl}} &   \multicolumn{3}{c|}{{\em qf\_shlid2\_entl}}  \\
 \hline
 & {\small \invalid} &  {\small \valid} & Time & {\small \invalid} &  {\small \valid} & Time & {\small \invalid} &  {\small \valid} & Time \\
    & {\small (122)} &  {\small (174)} & (296)  & {\small (24)} &  {\small (36)} &  (60) & {\small (14)} &  {\small (13)} & (27)  \\
\hline
SLS & 12 & 174 & 507m42s & 2 & 35 & 133m28s & 0 & 11 & 97m54s \\
\rowcolor{Gray} \spen & 122 & 174 & 10.78s & 14 & 13 & 3.44s & 8 & 2 & 1.69s\\
\cyclic & 0 & 58 & 1520m5s & 0 & 24 & 360m38s & 0 & 3 & 240m3s \\
\rowcolor{Gray} \harr & 39 & 116 & 425m19s & 18 & 27 & 53m56s & 8 & 7 & 156m45s \\
 \songbird & 12 & 174 & 237m25s & 2 & 35 & 40m38s & 0 & 12 & 47m11s \\
\rowcolor{Gray}\toolname & 122  & 174 & 6.22s & 24  & 36 & 0.96s & 14 & 13 & 1.20s \\
\hline
 \end{tabular}
\end{center}
\end{table}

